Improving Proper Noun Recognition in End-to-End ASR By Customization of the MWER Loss Criterion

Proper nouns present a challenge for end-to-end (E2E) automatic speech recognition (ASR) systems in that a particular name may appear only rarely during training, and may have a pronunciation similar to that of a more common word. Unlike conventional ASR models, E2E systems lack an explicit pronounciation model that can be specifically trained with proper noun pronounciations and a language model that can be trained on a large text-only corpus. Past work has addressed this issue by incorporating additional training data or additional models. In this paper, we instead build on recent advances in minimum word error rate (MWER) training to develop two new loss criteria that specifically emphasize proper noun recognition. Unlike past work on this problem, this method requires no new data during training or external models during inference. We see improvements ranging from 2% to 7% relative on several relevant benchmarks.

==> Main <==
\begin{thebibliography}{10}

\bibitem{Vu14}
Ngoc~Thang Vu, Yuanfan Wang, Marten Klose, Zlatka Mihaylova, and Tanja Schultz,
\newblock ``{Improving ASR Performance On Non-native Speech Using Multilingual
  and Crosslingual Information},'' 2014.

\bibitem{Shor19}
Joel Shor, Dotan Emanuel, Oran Lang, Omry Tuval, Michael Brenner, Julie
  Cattiau, Fernando Vieira, Maeve McNally, Taylor Charbonneau, Melissa
  Nollstadt, Avinatan Hassidim, and Yossi Matias,
\newblock ``Personalizing asr for dysarthric and accented speech with limited
  data,'' 2019.

\bibitem{Jain18}
Abhinav Jain, Minali Upreti, and Preethi Jyothi,
\newblock ``{Improved Accented Speech Recognition Using Accent Embeddings and
  Multi-task Learning},'' 2018.

\bibitem{Schultz00}
Tanja Schultz and A.~Waibel,
\newblock ``Multilingual and crosslingual speech recognition,''
\newblock 08 2000.

\bibitem{Hu19}
Ke~Hu, Antoine Bruguier, Tara~N. Sainath, Rohit Prabhavalkar, and Golan Pundak,
\newblock ``Phoneme-based contextualization for cross-lingual speech
  recognition in end-to-end models,'' 2019.

\bibitem{Vasserman15}
Keith~Hall Lucy~Vasserman, Vlad~Schogol,
\newblock ``Sequence-based class tagging for robust transcription in asr,''
\newblock in {\em INTERSPEECH}, 2015.

\bibitem{Peyser19}
Cal Peyser, Hao Zhang, Tara~N. Sainath, and Zelin Wu,
\newblock ``Improving performance of end-to-end asr on numeric sequences,''
  2019.

\bibitem{Beaufays03}
F.~{Beaufays}, A.~{Sankar}, S.~{Williams}, and M.~{Weintraub},
\newblock ``Learning name pronunciations in automatic speech recognition
  systems,''
\newblock in {\em Proceedings. 15th IEEE International Conference on Tools with
  Artificial Intelligence}, Nov 2003, pp. 233--240.

\bibitem{Laurent10}
Antoine Laurent, Sylvain Meignier, Teva Merlin, and Paul Deléglise,
\newblock ``Acoustics-based phonetic transcription method for proper nouns,''
\newblock 01 2010, pp. 2286--2289.

\bibitem{Graves12}
Alex Graves,
\newblock ``Sequence transduction with recurrent neural networks,'' 2012.

\bibitem{Chan15}
William Chan, Navdeep Jaitly, Quoc~V. Le, and Oriol Vinyals,
\newblock ``Listen, attend and spell,'' 2015.

\bibitem{He18}
Yanzhang He, Tara~N. Sainath, Rohit Prabhavalkar, Ian McGraw, Raziel Alvarez,
  Ding Zhao, David Rybach, Anjuli Kannan, Yonghui Wu, Ruoming Pang, Qiao Liang,
  Deepti Bhatia, Yuan Shangguan, Bo~Li, Golan Pundak, Khe~Chai Sim, Tom Bagby,
  Shuo{-}Yiin Chang, Kanishka Rao, and Alexander Gruenstein,
\newblock ``Streaming end-to-end speech recognition for mobile devices,''
\newblock {\em CoRR}, vol. abs/1811.06621, 2018.

\bibitem{Alon19}
U.~{Alon}, G.~{Pundak}, and T.~N. {Sainath},
\newblock ``Contextual speech recognition with difficult negative training
  examples,''
\newblock in {\em ICASSP 2019 - 2019 IEEE International Conference on
  Acoustics, Speech and Signal Processing (ICASSP)}, May 2019, pp. 6440--6444.

\bibitem{Prabhavalkar17}
Rohit Prabhavalkar, Tara~N. Sainath, Yonghui Wu, Patrick Nguyen, Zhifeng Chen,
  Chung{-}Cheng Chiu, and Anjuli Kannan,
\newblock ``Minimum word error rate training for attention-based
  sequence-to-sequence models,''
\newblock {\em CoRR}, vol. abs/1712.01818, 2017.

\bibitem{Shannon17}
Matt Shannon,
\newblock ``Optimizing expected word error rate via sampling for speech
  recognition,'' 2017.

\bibitem{Sainath19}
Tara~N. Sainath, Ruoming Pang, David Rybach, Yanzhang He, Rohit Prabhavalkar,
  Wei Li, Mirkó Visontai, Qiao Liang, Trevor Strohman, Yonghui Wu, Ian McGraw,
  and Chung-Cheng Chiu,
\newblock ``Two-pass end-to-end speech recognition,'' 2019.

\bibitem{Kim17}
Chanwoo Kim, Ananya Misra, Kean Chin, Thad Hughes, Arun Narayanan, Tara
  Sainath, and Michiel Bacchiani,
\newblock ``Generation of large-scale simulated utterances in virtual rooms to
  train deep-neural networks for far-field speech recognition in google home,''
\newblock 08 2017, pp. 379--383.

\bibitem{Gonzalvo16}
Xavi Gonzalvo, Siamak Tazari, Chun an~Chan, Markus Becker, Alexander Gutkin,
  and Hanna Sil{\'e}n,
\newblock ``Recent advances in google real-time hmm-driven unit selection
  synthesizer,''
\newblock in {\em INTERSPEECH}, 2016.

\bibitem{Pundak16}
Golan Pundak and Tara~N. Sainath,
\newblock ``Lower frame rate neural network acoustic models,''
\newblock in {\em INTERSPEECH}, 2016.

\bibitem{Huang15}
Zhiheng Huang, Wei Xu, and Kai Yu,
\newblock ``Bidirectional lstm-crf models for sequence tagging,'' 2015.

\bibitem{Hixon11}
Ben Hixon, Eric Schneider, and Susan Epstein,
\newblock ``Phonemic similarity metrics to compare pronunciation methods.,''
\newblock 01 2011, pp. 825--828.

\end{thebibliography}

